On the Mitigation of Read Disturbances in Neuromorphic Inference Hardware

Non-Volatile Memory (NVM) cells are used in neuromorphic hardware to store model parameters, which are programmed as resistance states. NVMs suffer from the read disturb issue, where the programmed resistance state drifts upon repeated access of a cell during inference. Resistance drifts can lower the inference accuracy. To address this, it is necessary to periodically reprogram model parameters (a high overhead operation). We study read disturb failures of an NVM cell. Our analysis show both a strong dependency on model characteristics such as synaptic activation and criticality, and on the voltage used to read resistance states during inference. We propose a system software framework to incorporate such dependencies in programming model parameters on NVM cells of a neuromorphic hardware. Our framework consists of a convex optimization formulation which aims to implement synaptic weights that have more activations and are critical, i.e., those that have high impact on accuracy on NVM cells that are exposed to lower voltages during inference. In this way, we increase the time interval between two consecutive reprogramming of model parameters. We evaluate our system software with many emerging inference models on a neuromorphic hardware simulator and show a significant reduction in the system overhead.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> sections/neuromorphic.tex <==



In this section, we briefly introduce neuromorphic computing, focusing on Spiking Neural Network (SNN)-based machine learning tasks and their implementation in hardware.

\subsection{Machine Learning Inference}
Spiking Neural Networks (SNNs) are emerging computation models designed using spiking neurons and bio-inspired learning algorithms~\cite{maass1997networks}. Spiking neurons are connected via the synapses. The left subfigure of Figure~\ref{fig:snn} shows an SNN, where the neurons are connected in a feedforward topology.
Information in SNNs is encoded into spike trains, which capture the spatio-temporal properties of input data. 
The right subfigure of Fig.~\ref{fig:snn} shows the spike communication from a pre-synaptic neuron to a post-synaptic neuron via a synapse. 


\begin{figure}[h!]
	\begin{center}
		\vspace{-10pt}
		%\includegraphics[width=5.75in]{./image/proposal.pdf}
		\includegraphics[width=0.99\columnwidth]{images/snn.pdf}
		\vspace{-10pt}
		\caption{Spiking neural network}
		%\vspace{-10pt}
		\label{fig:snn}
		\vspace{-10pt}
	\end{center}
\end{figure}

SNNs can implement many different machine learning approaches such as supervised, unsupervised, reinforcement, few-shot, and lifelong learning. 
Supervised learning is the primary focus of this work. In supervised learning, a model is trained with representative training data, where training refers to adjusting the weights of synaptic connections to reduce the error between the expected and actual output. Machine learning inference refers to feeding live data points to this trained model for generating output.

\subsection{Architecture of Neuromorphic Hardware}
A neuromorphic hardware platform is implemented as a tiled architecture, where tiles are interconnected via a time-multiplexed shared interconnect.
Each tile consists of a neuromorphic processing element (PE), which can implement neurons and synapses of a machine learning model.
 A common design practice is to use analog crossbars to implement a PE.

In a crossbar, pre-synaptic neuron circuits are placed on horizontal wires called wordlines, while post-synaptic neuron circuits are placed on vertical wires called bitlines. Memory cells are placed at the crosspoint of each wordline and bitline, and they implement the synaptic weights of an SNN. The left subfigure of Figure~\ref{fig:crossbar} illustrates an $N \times N$ crossbar. The right subfigure illustrates the parasitic RC components on the current path from a pre-synaptic neuron to a post-synaptic neuron accessing the memory cell $(i,j)$ located at the crosspoint of \ineq{i^\text{th}} wordline and \ineq{j^\text{th}} bitline.

\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/crossbar.pdf}}
	\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{An $N \times N$ crossbar showing the parasitic components within.}
	\vspace{-5pt}
	\label{fig:crossbar}
\end{figure}

Formally, the number of parasitic components on the current path via the $(i,j)^\text{th}$ memory cell is $(i+j+1)$.





Figure~\ref{fig:current_variation} shows the current variation in a crossbar at four different process technology nodes. We show the current through memory cell at positions $(0,0)$ and $(N-1,N-1)$ in the crossbar. We make the following two observations.

\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/current_variation.pdf}}
	\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Current variation in a crossbar at different process technology nodes.}
	\vspace{-5pt}
	\label{fig:current_variation}
\end{figure}

First, the current through a crossbar reduces with technology scaling. This is due to the increase in the size of the parasitics on bitlines and wordlines. 
The unit wordline (bitline) parasitic resistance ranges from approximately \ineq{2.5\Omega} (\ineq{1\Omega}) at {65nm} node to  \ineq{10\Omega} (\ineq{3.8\Omega}) at {16nm} node. The value of these unit parasitic resistances are expected to scale further reaching \ineq{\approx 25\Omega} at {5nm} node~\cite{espine}. The unit wordline and bitline capacitance values also scale proportionately with technology.
Second, the current variation in a crossbar becomes significant with technology scaling due to an increase in the size of parasitics at scaled process technology nodes.

\subsection{Implementing Machine Learning Inference on Neuromorphic Hardware}
To implement an SNN-based inference task on a neuromorphic hardware, the trained synaptic weights of the SNN are programmed on the memory cells of different crossbars in the hardware. To this end,
a crossbar can accommodate only a fixed number of pre-synaptic connections per post-synaptic neuron. Its dimension is typically constrained to reduce the energy consumption. Each post-synaptic neuron in an $N\times N$ crossbar can have a maximum fanin of $N$ pre-synaptic neurons. Therefore, to map an SNN that cannot be implemented on to a single crossbar, the SNN needs to be partitioned into clusters, where each cluster consists of a part of neurons and synapses of the original SNN.
Each cluster is then implemented on to a crossbar of the hardware.

Figure~\ref{fig:mapping} shows the implementation of a small SNN to a crossbar.
Synaptic weights \ineq{w_{1}} and \ineq{w_{2}} are programmed into the memory cells P1 and  P2, respectively. The output spike voltages, \ineq{v_1} from N1 and \ineq{v_2} from N2, inject current into the crossbar, which are obtained by multiplying a pre-synaptic neuron's output spike voltage with the memory cell's conductance at the crosspoint of the pre- and post-synaptic neuron (following Ohm's law). Current summations along columns (bitlines) are performed in parallel using Kirchhoff’s current law, and implement the sums $\sum_j w_{i}v_i$, needed for forward propagation of neuron excitation.


\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.99\columnwidth]{images/mapping.pdf}}
	\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{Implementation of an SNN to a crossbaar.}
	\vspace{-5pt}
	\label{fig:mapping}
\end{figure}

==> sections/system_level.tex <==






A system-level approach to mitigating read disturbance issues in OxRRAM-based neuromorphic hardware is to periodically reprogram the trained weights in the hardware when executing an inference task. When such reprogramming is occurring, the hardware is unavailable to perform any inference task. Therefore, the system overhead of periodic reprogramming of neuromorphic is given by
\begin{equation}
    \label{eq:reprogramming_overhead}
    \footnotesize \text{reprogram overhead} = \frac{tRPT}{tRPI},
\end{equation}
where \ineq{tRPT} is defined as the reprogramming time, which is the time it takes to reprogram the synaptic weights of a machine learning model on neuromorphic hardware, and \ineq{tRPI} is the reprogram interval, which is defined as the time interval between two consecutive reprogram operations. \ineq{tRPI} is computed as the maximum of the transition capacities of the utilized OxRRAM cells in a crossbar.
%Our \textbf{objective} is to reduce the reprogram overhead by increasing the \ineq{tRPI}.

Figure~\ref{fig:framework} illustrates our system software framework based on NeuroXplorer~\cite{neuroxplorer} to incorporate read disturbance models in reprogramming the hardware. 
\begin{figure}[h!]
	\centering
	\vspace{-5pt}
	\centerline{\includegraphics[width=0.89\columnwidth]{images/framework.pdf}}
	\vspace{-10pt}
	%\caption{An example of spiking neural network.}
	\caption{System software framework based on NeuroXplorer~\cite{neuroxplorer}.}
	\vspace{-5pt}
	\label{fig:framework}
\end{figure}

The new components needed to mitigate read disturbance issues are shown in red. A machine learning model is first trained using representative training data. The trained data is then partitioned to generate clusters , where each cluster can be implemented on a crossbar. The clusters are inserted in a queue (\texttt{clQ}). In the baseline design, each cluster of the clQ is mapped onto an $N\times N$ crossbar array and the mapping is then implemented on hardware. To mitigate read disturbance issues, circuit-level models are used to determine the reprogram interval for a given mapping. An internal counter is maintained, which is set to the reprogram interval. The counter is decremented every time an inference operation is performed by the hardware. When the counter expires, the trained wights are reprogrammed to the hardware and the counter is set to the reprogram interval again. In this way, the system software ensures that the hardware is programmed periodically every reprogram interval.







